Image-to-Lidar Relational Distillation for Autonomous Driving Data

Pre-trained on extensive and diverse multi-modal datasets, 2D foundation models excel at addressing 2D tasks with little or no downstream supervision, owing to their robust representations. The emergence of 2D-to-3D distillation frameworks has extended these capabilities to 3D models. However, distilling 3D representations for autonomous driving datasets presents challenges like self-similarity, class imbalance, and point cloud sparsity, hindering the effectiveness of contrastive distillation, especially in zero-shot learning contexts. Whereas other methodologies, such as similarity-based distillation, enhance zero-shot performance, they tend to yield less discriminative representations, diminishing few-shot performance. We investigate the gap in structure between the 2D and the 3D representations that result from state-of-the-art distillation frameworks and reveal a significant mismatch between the two. Additionally, we demonstrate that the observed structural gap is negatively correlated with the efficacy of the distilled representations on zero-shot and few-shot 3D semantic segmentation. To bridge this gap, we propose a relational distillation framework enforcing intra-modal and cross-modal constraints, resulting in distilled 3D representations that closely capture the structure of the 2D representation. This alignment significantly enhances 3D representation performance over those learned through contrastive distillation in zero-shot segmentation tasks. Furthermore, our relational loss consistently improves the quality of 3D representations in both in-distribution and out-of-distribution few-shot segmentation tasks, outperforming approaches that rely on the similarity loss.

==> content/tables.tex <==



% CLIP backbones with contrastive losses
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{CLIP backbones}
\centering
\begin{tabular}{clrrrrrrr}
\toprule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}2D \\ Encoder\end{tabular}} & \multicolumn{1}{c}{\multirow{3}{*}{Loss}} & \multicolumn{1}{c}{\multirow{3}{*}{Uniformity}} & \multicolumn{1}{c}{\multirow{3}{*}{Tolerance}} & \multicolumn{1}{c}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Modality \\ Gap\end{tabular}}} & \multicolumn{3}{c}{nuScenes}                                                                                                                                                                                               & \multicolumn{1}{c}{KITTI}                                                             \\ \cline{6-9} 
                                                                       & \multicolumn{1}{c}{}                      & \multicolumn{1}{c}{}                            & \multicolumn{1}{c}{}                           & \multicolumn{1}{c}{}                                                                         & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}LP\\ 100\%\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}{*}{ZS}} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Ft\\  1\%\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Ft\\ 1\%\end{tabular}}} \\
                                                                       & \multicolumn{1}{c}{}                      & \multicolumn{1}{c}{}                            & \multicolumn{1}{c}{}                           & \multicolumn{1}{c}{}                                                                         & \multicolumn{1}{c}{}                                                                    & \multicolumn{1}{c}{}                    & \multicolumn{1}{c}{}                                                                   & \multicolumn{1}{c}{}                                                                  \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{ViT-B32}}                          & PPKT                                      & 3.511                                           & 0.5203                                         & 0.0002                                                                                       & \underline{45.96}                                                                                   & 14.21                                   & 43.29                                                                                  & \textbf{45.89}                                                                                 \\
\multicolumn{1}{c|}{}                                                  & Sim-pt                                    & 0.5804                                          & 0.9389                                         & 0.0001                                                                                       & 45.41                                                                                   & 22.84                                   & 44.22                                                                                  & 44.30                                                                                 \\
\multicolumn{1}{c|}{}                                                  & Rel$_{pt}$                                       & 0.9605                                          & 0.8989                                         & \textbf{0.0001}                                                                                       & \textbf{46.06}                                                                                   & \textbf{23.85}                                   & \textbf{44.67}                                                                                  & \underline{45.62}                                                                                 \\ \cline{2-9} 
\multicolumn{1}{c|}{}                                                  & SLidR                                     & 3.513                                           & 0.4706                                         & 0.0003                                                                                       & \textbf{48.73}                                                                                   & 15.55                                   & 43.38                                                                                  & 43.82                                                                                 \\
\multicolumn{1}{c|}{}                                                  & Sim$_{sp}$                                    & 0.6009                                          & 0.9323                                         & 0.00011                                                                                      & 47.26                                                                                   & \underline{25.46}                                   & \underline{44.83}                                                                                  & \underline{45.69}                                                                                 \\
\multicolumn{1}{c|}{}                                                  & Rel$_{sp}$                                    & 1.202                                           & 0.8648                                         & \textbf{0.00007}                                                                                      & \underline{48.00}                                                                                   & \textbf{25.66}                                   & \textbf{45.60}                                                                                  & \textbf{47.26}                                                                                 \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{VIT-B16}}                          & PPKT                                      & 3.521                                           & 0.5217                                         & 0.001582                                                                                     & \textbf{50.54}                                                                                   & 14.53                                   & \underline{45.31}                                                                                  & \underline{45.77}                                                                                 \\
\multicolumn{1}{c|}{}                                                  & Sim-pt                                    & 0.5519                                          & 0.9477                                         & \underline{0.00045}                                                                                      & 49.70                                                                                   & \underline{20.84}                                   & 44.39                                                                                  & 45.59                                                                                 \\
\multicolumn{1}{c|}{}                                                  & Rel$_{pt}$                                       & 0.9089                                          & 0.9145                                         & \textbf{0.00033}                                                                                      & \underline{50.33}                                                                                   & \textbf{23.53}                                   & \textbf{45.67}                                                                                  & \textbf{46.06}                                                                                 \\ \cline{2-9} 
\multicolumn{1}{c|}{}                                                  & SLidR                                     & 3.509                                           & 0.4472                                         & 0.00153                                                                                      & \textbf{51.88}                                                                                   & 16.82                                   & \underline{46.76}                                                                                  & \underline{46.53}                                                                                 \\
\multicolumn{1}{c|}{}                                                  & Sim$_{sp}$                                    & 0.5919                                          & 0.9333                                         & \underline{0.0004}                                                                                       & 50.28                                                                                   & \underline{23.93}                                   & 45.63                                                                                  & 46.42                                                                                 \\
\multicolumn{1}{c|}{}                                                  & Rel$_{sp}$                                    & 1.099                                           & 0.87                                           & \textbf{0.00019}                                                                                      & \underline{50.40}                                                                                   & \textbf{26.03}                                   & \textbf{47.22}                                                                                  & \textbf{47.52}                                                                                 \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{ViT-L14}}                          & PPKT                                      & 3.502                                           & 0.5203                                         & 0.00089                                                                                      & \textbf{51.08}                                                                                   & 16.28                                   & 44.69                                                                                  & \textbf{46.69}                                                                                 \\
\multicolumn{1}{c|}{}                                                  & Sim$_{pt}$                                   & 0.6909                                          & 0.9257                                         & \underline{0.00016}                                                                                      & 49.76                                                                                   & \textbf{27.91}                                   & \underline{44.87}                                                                                  & 44.80                                                                                 \\
\multicolumn{1}{c|}{}                                                  & Rel$_{pt}$                                       & 0.8775                                          & 0.9027                                         & \textbf{0.00013}                                                                                      & \underline{50.64}                                                                                   & \underline{27.74}                                   & \textbf{45.92}                                                                                  & \underline{45.86}                                                                                 \\ \cline{2-9} 
\multicolumn{1}{c|}{}                                                  & SLidR                                     & 3.48                                            & 0.4403                                         & 0.00065                                                                                      & 51.46                                                                                   & 18.31                                   & \textbf{47.34}                                                                                  & \textbf{46.86}                                                                                 \\
\multicolumn{1}{c|}{}                                                  & Sim$_{sp}$                                    & 0.7311                                          & 0.9102                                         & \underline{0.0002}                                                                                       & 49.35                                                                                   & \textbf{30.77}                                   & 45.76                                                                                  & 45.29                                                                                 \\
\multicolumn{1}{c|}{}                                                  & Rel$_{sp}$                                    & 0.9019                                          & 0.8873                                        & \textbf{0.00017}                                                                                      & \underline{49.54}                                                                                   & \underline{30.11}                                   & \underline{47.07}                                                                                  & \underline{46.81}  \\
\bottomrule
\end{tabular}
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Main Results on CLIP (ViT-B16) and DINOv2. $pt$ refers to pixel-point and $sp$ refers to superpixel-superpoint distillation. CLIP image encoder uniformity is 1.54, and tolerance is 0.73. DINOv2 image encoder uniformity is 2.8 and tolerance is 0.51}
\centering
\begin{tabular}{clrrrrrrr}
\toprule

\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}2D \\ Encoder\end{tabular}} & \multicolumn{1}{c}{\multirow{3}{*}{Loss}} & \multicolumn{1}{c}{\multirow{3}{*}{Uniformity}} & \multicolumn{1}{c}{\multirow{3}{*}{Tolerance}} & \multicolumn{1}{c}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Modality\\  Gap\end{tabular}}} & \multicolumn{3}{c}{nuScenes}                                                                                                                                                                                                                       & \multicolumn{1}{c}{KITTI}                                                                    \\ \cline{6-9} 
                                                                     & \multicolumn{1}{c}{}                      & \multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                      & \multicolumn{1}{c}{}                                                                         & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}LP. \\ 100\%\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}{*}{ZS}} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Ft \\ 1\%\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Ft \\ 1\%\end{tabular}}} \\
                                                                     & \multicolumn{1}{c}{}                      & \multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                      & \multicolumn{1}{c}{}                                                                         & \multicolumn{1}{c}{}                                                                               & \multicolumn{1}{c}{}                           & \multicolumn{1}{c}{}                                                                         & \multicolumn{1}{c}{}                                                                         \\ \hline
\multicolumn{1}{c|}{\multirow{7}{*}{CLIP~\cite{radford2021learningclip}}}                           & PPKT~\cite{liu2021ppkt}                                      & 3.521                                      & 0.5217                                    & 0.0016                                                                                       & \textbf{50.54}                                                                                              & 14.53                                          & \underline{45.31}                                                                                        & \underline{45.77}                                                                                        \\
\multicolumn{1}{c|}{}                                                & Sim$_{pt}$                                 & 0.5519                                     & 0.9477                                    & 0.00045                                                                                      & 49.70                                                                                              & \underline{20.84}                                          & 44.39                                                                                        & 45.59                                                                                        \\
\multicolumn{1}{c|}{}                                                & Rel$_{pt}$                                 & 0.9089                                     & 0.9145                                    & \textbf{0.00033}                                                                                      & 50.33                                                                                              & \textbf{23.53}                                          & \textbf{45.67}                                                                                        & \textbf{46.06}                                                                                        \\ \cline{2-9} 
\multicolumn{1}{c|}{}                                                & SLidR~\cite{sautier2022slidr, liu2023seal}                                     & 3.509                                      & 0.4472                                    & 0.00153                                                                                      & \underline{51.88}                                                                                              & 16.82                                          & 46.76                                                                                        & 46.53                                                                                        \\
\multicolumn{1}{c|}{}                                                & ST-SLidR~\cite{stcl}                                  & 3.5                                        & 0.4544                                    & 0.0015                                                                                       & \textbf{52.05}                                                                                              & 18.54                                          & \underline{47.13}                                                                                        & \underline{46.84}                                                                                        \\
\multicolumn{1}{c|}{}                                                & Sim$_{sp}$                                    & 0.5919                                     & 0.9333                                    & 0.0004                                                                                       & 50.28                                                                                              & 23.93                                          & 45.63                                                                                        & 46.42                                                                                        \\
\multicolumn{1}{c|}{}                                                & Rel$_{sp}$                                    & 1.099                                      & 0.87                                      & \textbf{0.00019}                                                                                       & 50.40                                                                                              & \textbf{26.03}                                          & \textbf{47.22}                                                                                        & \textbf{47.52}                                                                                        \\ \hline
\multicolumn{1}{c|}{\multirow{7}{*}{DINOv2~\cite{oquab2023dinov2}}}                         & PPKT~\cite{liu2021ppkt}                                      & 3.625                                      & 0.4451                                    & 0.0006                                                                                       & 48.50                                                                                              & N/A                                            & 43.30                                                                                        & 43.62                                                                                        \\
\multicolumn{1}{c|}{}                                                & Sim$_{pt}$                                 & 2.176                                      & 0.6926                                    & 0.0003                                                                                       & \textbf{49.72}                                                                                              & N/A                                            & \underline{45.85}                                                                                        & \underline{48.32}                                                                                        \\
\multicolumn{1}{c|}{}                                                & Rel$_{pt}$                                 & 2.393                                      & 0.6588                                    & \textbf{0.0002}                                                                                       & \underline{49.20}                                                                                              & N/A                                            & \textbf{46.90}                                                                                        & \textbf{49.00}                                                                                        \\ \cline{2-9} 
\multicolumn{1}{c|}{}                                                & SLidR~\cite{sautier2022slidr, liu2023seal}                                     & 3.655                                      & 0.3739                                    & 0.00044                                                                                      & 49.60                                                                                              & N/A                                            & 44.81                                                                                        & 42.23                                                                                        \\
\multicolumn{1}{c|}{}                                                & ST-SLidR~\cite{stcl}                                  & 3.589                                      & 0.4326                                    & 0.00042                                                                                      & \textbf{53.00}                                                                                              & N/A                                            & 47.11                                                                                        & 45.61                                                                                        \\
\multicolumn{1}{c|}{}                                                & Sim$_{sp}$                                    & 2.286                                      & 0.6522                                    & \underline{0.0003}                                                                                       & 52.30                                                                                              & N/A                                            & \underline{47.23}                                                                                        & \underline{49.01}                                                                                        \\
\multicolumn{1}{c|}{}                                                & Rel$_{sp}$                                    & 2.504                                      & 0.6312                                    & \textbf{0.0002}                                                                                       & \underline{52.92}                                                                                              & N/A                                            & \textbf{48.42}                                                                                        & \textbf{49.10}     \\
\bottomrule
\end{tabular}
%\label{tab:main_results_reference}
\end{table}


% Evaluate majority versus minority class improvements
\begin{table}[]
\caption{Evaluating improvement of finetuned models on majority and minority classes of nuScenes dataset.}
\begin{tabular}{clrr}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}2D \\ Encoder\end{tabular}} & \multicolumn{1}{c}{\multirow{2}{*}{Loss}} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Majority\\  (mIoU)\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Minority \\ (mIoU)\end{tabular}}} \\
                                                                       & \multicolumn{1}{c}{}                      & \multicolumn{1}{c}{}                                                                            & \multicolumn{1}{c}{}                                                                            \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{CLIP}}                             & Sim-pt                                    & 69.16                                                                                           & 33.35                                                                                           \\
\multicolumn{1}{c|}{}                                                  & Rel-pt                                    & 69.59                                                                                           & 34.80                                                                                           \\
\multicolumn{1}{c|}{}                                                  & Gain                                      & 0.43                                                                                            & 1.45                                                                                            \\ \cline{2-4} 
\multicolumn{1}{c|}{}                                                  & Sim-sp                                    & 67.58                                                                                           & 36.06                                                                                           \\
\multicolumn{1}{c|}{}                                                  & Rel-sp                                    & 67.75                                                                                           & 38.77                                                                                           \\
\multicolumn{1}{c|}{}                                                  & Gain                                      & 0.17                                                                                            & 2.71                                                                                            \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{DINOv2}}                           & Sim-pt                                    & 70.89                                                                                           & 34.24                                                                                           \\
\multicolumn{1}{c|}{}                                                  & Rel-pt                                    & 71.22                                                                                           & 35.85                                                                                           \\
\multicolumn{1}{c|}{}                                                  & Gain                                      & 0.33                                                                                            & 1.61                                                                                            \\ \cline{2-4} 
\multicolumn{1}{c|}{}                                                  & Sim-sp                                    & 68.15                                                                                           & 38.53                                                                                           \\
\multicolumn{1}{c|}{}                                                  & Rel-sp                                    & 68.80                                                                                           & 40.20                                                                                           \\
\multicolumn{1}{c|}{}                                                  & Gain                                      & 0.65                                                                                            & 1.67      \\
\bottomrule
\end{tabular}
\end{table}


% loss ablations
\begin{table}[]
\centering
\caption{Ablation studies for point-based and superpoint-based relational loss. Source uniformity and tolerance are 1.54 and 0.73 respectively.}
\begin{tabular}{lrrrrrrr}
\toprule
\multicolumn{1}{c}{\multirow{3}{*}{Loss}} & \multicolumn{1}{c}{\multirow{3}{*}{Uniformity}} & \multicolumn{1}{c}{\multirow{3}{*}{Tolerance}} & \multicolumn{1}{c}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Modality \\ Gap\end{tabular}}} & \multicolumn{3}{c}{nuScenes}                                                                                                                                                                                               & \multicolumn{1}{c}{KITTI}                                                             \\ \cline{5-8} 
\multicolumn{1}{c}{}                      & \multicolumn{1}{c}{}                            & \multicolumn{1}{c}{}                           & \multicolumn{1}{c}{}                                                                         & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}LP\\ 100\%\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}{*}{ZS}} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Ft \\ 1\%\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Ft\\ 1\%\end{tabular}}} \\
\multicolumn{1}{c}{}                      & \multicolumn{1}{c}{}                            & \multicolumn{1}{c}{}                           & \multicolumn{1}{c}{}                                                                         & \multicolumn{1}{c}{}                                                                    & \multicolumn{1}{c}{}                    & \multicolumn{1}{c}{}                                                                   & \multicolumn{1}{c}{}                                                                  \\ \hline
Sim$_{pt}$                                   & 0.5519                                          & 0.9477                                         & 0.00045                                                                                      & 49.70                                                                                   & 20.84                                   & 44.39                                                                                  & 45.59                                                                                 \\
\tiny{+cross-modal}                                    & 0.6426                                          & 0.9386                                         & 0.00042                                                                                      & 49.87                                                                                   & 21.39                                  & \textbf{45.95}                                                                                  & 45.45                                                                                 \\
\tiny{+uni-modal}                                 & 0.9089                                          & 0.9145                                         & \textbf{0.00033}                                                                                      & \textbf{50.33}                                                                                   & \textbf{23.53}                                   & 45.67                                                                                  & \textbf{46.06}                                                                                 \\ \hline
Sim$_{sp}$                                   & 0.5919                                          & 0.9333                                         & 0.0004                                                                                       & 50.28                                                                                   & 23.93                                   & 45.63                                                                                  & 46.42                                                                                 \\
\tiny{+cross-modal}                                    & 0.7656                                          & 0.9086                                         & 0.00033                                                                                      & 50.26                                                                                   & 25.05                                   & 46.18                                                                                  & 46.99                                                                                 \\
\tiny{+uni-modal}                                 & 1.099                                           & 0.87                                           & \textbf{0.00019}                                                                                      & \textbf{50.40}                                                                                   & \textbf{26.03}                                   & \textbf{47.22}                                                                                  & \textbf{47.52}   \\
\bottomrule
\end{tabular}
\end{table}

% label-free performance
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Performance of Relational loss compared to state-of-the-art label-free segmentation methods}
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Publication} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Class Names \\ Required\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Use \\ SAM\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}3D \\ mIoU\end{tabular}} \\
                        &                              &                                                                                  &                                                                            &                          \\ \hline
MaskCLIP~\cite{zhou2022extractMaskCLIP}                & ECCV 2022                     & No                                                                               & No                                                                         & 12.80                    \\
OpenScene~\cite{peng2023openscene}               & CVPR 2023                     & No                                                                               & No                                                                         & 14.60                    \\
CLIP2Scene~\cite{chen2023clip2scene}              & CVPR 2023                     & Yes                                                                              & No                                                                         & 20.80                    \\
\text{Rel}$_{pt}$ (ours)          & -                            & No                                                                               & No                                                                         & 23.53                    \\ \hline
Towards~\cite{chen2023towards}                 & NeurIPS 2023                  & Yes                                                                              & Yes                                                                        & 26.80                    \\
\text{Rel}$_{sp}$ (ours)          & -                            & No                                                                               & Yes                                                                        & 26.03    
\\
\bottomrule
\end{tabular}
% \label{tab:sota_zeroshot}
\end{table}
